Decentralized Multi-Party Multi-Network AI for Global Deployment of 6G Wireless Systems

Multiple visions of 6G networks elicit Artificial Intelligence (AI) as a central, native element. When 6G systems are deployed at a large scale, end-to-end AI-based solutions will necessarily have to encompass both the radio and the fiber-optical domain. This paper introduces the Decentralized Multi-Party, Multi-Network AI (DMMAI) framework for integrating AI into 6G networks deployed at scale. DMMAI harmonizes AI-driven controls across diverse network platforms and thus facilitates networks that autonomously configure, monitor, and repair themselves. This is particularly crucial at the network edge, where advanced applications meet heightened functionality and security demands. The radio/optical integration is vital due to the current compartmentalization of AI research within these domains, which lacks a comprehensive understanding of their interaction. Our approach explores multi-network orchestration and AI control integration, filling a critical gap in standardized frameworks for AI-driven coordination in 6G networks. The DMMAI framework is a step towards a global standard for AI in 6G, aiming to establish reference use cases, data and model management methods, and benchmarking platforms for future AI/ML solutions.

==> sections/1.1-related_work.tex <==
\subsection{Related Work}
% Traditional mobile networks are based on monolithic and hardware-based \acp{ran}, which are inflexible and difficult to customize. However, the industry is moving towards more agile and innovative solutions based on softwarization, open interfaces, and disaggregation. 
Mobile networks are transitioning from monolithic, hardware-based and inflexible \acp{ran} towards agile and innovative solutions based on softwarization, open interfaces, and disaggregation. These new approaches allow for more flexible and customizable networks that can be optimized for specific needs. Current efforts towards 6G networks take this a step further by incorporating \ac{ai}-based control loops and exposing \acp{api} for \ac{ml}-based solutions. This will enable network operators to optimize network functionality from mobility to the \ac{phy} and \ac{mac} layers \cite{hoydis2021toward, 10008643}. Additionally, the O-RAN alliance is developing standards for AI-native networks, which will allow mobile operators to deploy standardized third-party \ac{ml} models to orchestrate their entire \ac{ran} \cite{polese2023understanding}. Specifically, O-RAN working group 2 is focused on developing \ac{ai} workflow architectures for network control within the O-RAN architecture.

As O-RAN specifications evolve, researchers are exploring its potential as a platform for embedding \ac{ai}/\ac{ml} workflows within the network \cite{giannopoulos2022supporting,lee2020hosting}. 
% These methods utilize xApps for near-\ac{rt} \acp{ric} and rApps for non-\ac{rt} \acp{ric}. 
O-RAN is collaborating with the ONAP and Acumos projects to integrate \ac{ai}-based tools into the O-RAN architecture \cite{ONAP2022}. 
% However, these tools are resource-intensive and not ideal for research purposes. 
Lightweight x/rApps have been developed for open-source \acp{ric} \cite{lee2020hosting, xavier2023machine}. Integration of \ac{ric}-based AI network controls with \ac{sdn} is also being explored \cite{donertasli2022disaggregated, xavier2024cross}. \ac{pai} and \ac{aiaas} approaches are being extended to the O-RAN \ac{ric} architecture \cite{baccour2023zero}. While the O-RAN architecture provides a standardized platform for \ac{ai}/\ac{ml} control in radio networks, there is no equivalent for transport and optical networks. These domains typically utilize \ac{sdn} platforms like \ac{onos} to orchestrate network functions \cite{akinrintoyo2023reconfigurable}. The \ac{tip} further brings in open cell gateway functions to the environment \cite{grammel2018physical}. Much of the \ac{ai} control in optical networks focuses on offline \ac{qot} estimation, wavelength routing, and fault management \cite{mata2018artificial}. Extensions of \ac{onos} for online \ac{ai} and hierarchical control have also been explored \cite{morro2018automated}. The application of \ac{ai} methods to network control operations is a relatively new area of research, particularly in the context of radio and optical networks. Hence, there 
is a lack of standardized frameworks and tools for cross-domain \ac{ai}-based control and developing those will be highly beneficial.  
% A consensus-driven framework on open platforms would facilitate collaboration and accelerate progress.

\ac{zsm} aims to automate the orchestration of network resources using techniques like \ac{ai}/\ac{ml}, game theory, and optimization, to pursue the 6G key performance indicators \cite{baccour2023zero}. However, existing orchestration solutions often lack the agility and automation required for seamless service deployment changes. 
ETSI recognizes \ac{ai}/\ac{ml} as a key enabler for enhanced automation, data access, information abstraction, supervision, and streamlined lifecycle management \cite{etsi2020zsm}. 
\ac{ai}/\ac{ml}-powered network optimization can operate across different timescales, enabling more intelligent orchestration capabilities beyond ETSI NFV MANO's current specifications. ETSI NFV MANO considers incorporating \ac{ai}/\ac{ml} for data feeding and action collection, but not for direct operation automation \cite{etsi2020zsm}. Current NFV MANO automation relies on rule-based auto-scaling and auto-healing policies triggered by performance conditions.
Recently, several promising approaches to creating decentralized zero-touch management frameworks for coping with 6G network dynamicity have been proposed, such as embedding \ac{pai} as a service in 6G ecosystems in \cite{baccour2023zero}, the introduction of decision-making entities into distributed network elements in \cite{chergui2022toward}, and deep reinforcement learning for \ac{uav} edge networks in \cite{grasso2022smart}.
% , and deep Q-network algorithms for resource allocation in \cite{fu2020ai}. 
However, deploying \ac{ai}/\ac{ml} models in wireless networks is challenging due to dynamic topologies and the need for retraining with topology changes. Additionally, the complexity of decision-making and the requirement for large datasets for training necessitate distributed \ac{ml} techniques. Despite these challenges, zero-touch service management holds immense potential for enhanced efficiency, reliability, and scalability in 6G networks, driving the need for further innovation and real-world testing.

To summarize, the integration of \ac{ai}/\ac{ml} into mobile network architectures is a crucial step towards developing next-generation networks that are not merely communication pipelines but also intelligent compute engines. This transformation requires a framework to enable the design and implementation of networks that can dynamically adapt to changing conditions, optimize resource utilization, and deliver enhanced performance. Such a framework will pave the way for a paradigm shift from communication-only networks to compute-and-communicate networks that can perform complex computations and make informed decisions in real-time.

\vspace{-0.5em}

==> sections/3-applicability.tex <==
\section{Framework Applicability}\label{sec:use-cases}
The usefulness of the \ac{dmmai} framework can only be fully grasped through the examination of diverse use cases. Here, we present multiple use cases that highlight the framework's capabilities and versatility. Additionally, we explore different ways to extend these use cases, demonstrating the framework's scalability and adaptability. By considering these examples, we gain a comprehensive understanding of \ac{dmmai}  framework's potential applications and its ability to address a wide range of challenges in various domains. 

\vspace{-0.5em}
\subsection{Zero-Touch AI Service Management and Orchestration}

\begin{figure}
    \centering
    \includegraphics[width=0.8\columnwidth]{figures/zero_touch_placement.pdf}
    \vspace{-3mm}
    \caption{High-level overview of zero-touch services placement in 6G.}\label{fig:high_level_overview_zero_touch_services_placement}
    \vspace{-3mm}
\end{figure}

Our framework empowers the development of decentralized, \ac{ai}-driven techniques for managing and orchestrating network services within 6G ecosystems. This approach not only enhances efficiency and scalability but also prioritizes addressing the diverse requirements of vertical industries, e.g., the automotive and transportation sectors. By leveraging \ac{ai}'s predictive and adaptive capabilities, our framework enables self-optimizing and self-healing network operations, minimizing human intervention and maximizing network performance, eventually leading to zero-touch \ac{ai} service management.

The complexity and heterogeneity of 6G networks demand a paradigm shift in network management, transitioning from traditional, manual methods to intelligent, automated orchestration. The \ac{sba} of 5G and beyond networks, with its virtualized network functions and application services, requires efficient and dynamic configuration and management. Current decision-making techniques, such as human intervention and rule-based algorithms, are often slow, error-prone, and inflexible. To address these limitations, our framework enables the development of \ac{ai}/\ac{ml}-powered orchestration solutions. By combining \ac{ai}/\ac{ml} with \ac{nfv}, containerization and \ac{sdn}, we can automate network management across multiple layers, from the \ac{ran} to the core network and data network (see Figure~\ref{fig:high_level_overview_zero_touch_services_placement}). This approach will enable real-time adaptation, optimization, and self-healing capabilities, ensuring optimal network performance and responsiveness to dynamic demands.

\begin{figure}
    \centering\includegraphics[width=0.9\columnwidth]{figures/zero_touch_service_management.pdf}
    \vspace{-3mm}
    \caption{Zero-touch Service Management anticipated in 6G to evaluate the utility of the DMMAI framework for delivering AIaaS.}\label{fig:zero_touch_services_management_anticipated}
    \vspace{-3mm}
\end{figure}

The \ac{dmmai} framework allows us to experiment with novel architectures, such as the \ac{meao} proof-of-concept solution implemented by the authors of \cite{slamnik2021collaborative}. \ac{meao} consists of loosely coupled management and orchestration elements. This architecture features open and programmable interfaces that enable communication between management and orchestration elements, fostering an intelligent and automated network management paradigm (i.e., zero-touch services). It can perform smart placement of vertical applications on distributed \ac{mec} nodes, in which it implements a quality-aware placement mechanism to select the optimal node to host the vertical application. Another functionality of \ac{meao} is to perform vertical application state migration from nodes belonging to different \ac{mec} domains. 
% The mechanism works in a proactive manner by triggering the state migration before crossing \ac{nfv} domains or cross-\ac{mno} domains. 
% In addition, \ac{meao} can control the applications running by scaling up/down as well as by performing their termination.

The \ac{meao} orchestration environment leverages a decentralized, multi-network, and multi-agent approach to achieve intelligent management and orchestration for 6G edge networks. Intelligent placement mechanisms continuously monitor network activity and make proactive decisions to reconfigure network resources and optimize network efficiency. This approach enables the development of sustainable 6G edge networks by deploying zero-touch services across both aerial and terrestrial edge environments. However, as 6G networks become more sophisticated, the requirements for intelligence and automation will continue to escalate. 6G will transform into a network of interconnected networks, necessitating a more pervasive and intensive integration of \ac{ai}/\ac{ml} techniques compared to previous generations. This implies that network intelligence will not be confined to the 6G edge but will permeate all network segments and encompass multiple radio access technologies, including LTE-U, 5G-NR, and Wi-Fi (as depicted in Figure~\ref{fig:zero_touch_services_management_anticipated}). To achieve this, decentralized \ac{ai} models must work in harmony to manage the network holistically, employing automated and intelligent approaches to optimize network resources, enhance energy efficiency, and ensure superior service quality. The \ac{dmmai} framework, with its \ac{aic} integration across diverse network nodes, enables such extensions and experimentation on the \ac{meao} platform, paving the way for innovative network management solutions.

\vspace{-0.5em}
\subsection{Distributed AI at different time scales}
The O-RAN architecture envisions a network where \ac{ran} components expose manageable parameters and performance metrics, allowing for fine-tuning based on operator goals, network conditions, and traffic patterns. This enables intelligent control using \ac{ai}/\ac{ml} algorithms. However, current O-RAN implementations focus on applying \ac{ai} to higher-layer protocols, limiting flexibility for lower-layer control at \acp{du} and \acp{ru}. This constraint hinders the utilization of data-driven solutions requiring real-time or sub-millisecond control decisions, such as scheduling and beam management in sub-THz communication. These challenges are expected to intensify with the introduction of sensing, localization, and vertical applications demanding real-time performance and reliability. To address these limitations, O-RAN architectures should evolve to support control decisions across different timescales, including real-time operation with control loops shorter than current capabilities~\cite{dealmeida2021}. This requires consideration of factors like data availability and quality, application requirements, geographical constraints, and network workload. To that end, respecting timing aspects while ensuring a level of statistical guarantees on the offered end-to-end services involves designing communication protocols that involve privacy-aware, multi-modal, multi-party knowledge and data acquisition methods at scale. This demands efficient integration/aggregation of distributed intelligence and information in network planning, management, control, and operation. Furthermore, efficient quality-aware data compression and management is needed due to vast amounts of data. 

Decentralizing the \ac{ric} architecture requires a balance between data availability and use-case-specific constraints, particularly in terms of latency and data quality. While data exchange between distributed \ac{ric} instances is essential, minimizing overhead and securing sensitive information are crucial considerations. Federated reinforcement learning, which enables cooperation without data sharing, offers a potential approach to address these challenges. The proposed \ac{dmmai} framework facilitates a platform to experiment with different strategies and measure the impact on the data exchange overhead, latency and data quality related to decision-making. The \ac{aic} architecture, with its modular design, allows us to quickly build prototypes of decentralized \ac{ai}-based decision entities and instantiate them within different network entities. This further allows us to design intelligent algorithms to rely only on the data available at different network nodes and at different protocol layers. 

\vspace{-1em}
\subsection{Security and Authentication}
The integration of \ac{ai}/\ac{ml} into the O-RAN architecture introduces new security challenges beyond the ethical concerns associated with \ac{ai}/\ac{ml}, such as potential biases and data privacy issues. A significant concern is the reliance on third-party \ac{ml} models for zero-touch network management could open up vulnerabilities to malicious agents through the distribution of models via the public Internet. Phishing and \ac{dns} spoofing techniques can redirect legitimate model requests to repositories of malicious models, which can disrupt network performance in various ways. These malicious models can be (i) hampered by fine-tuning or retraining with intentionally flawed data, (ii) impersonated by counterfeit models that appear legitimate but provide inaccurate results, or (iii) neural trojans that function like genuine models but secretly incorporate malicious code without affecting system performance, making them difficult to detect~\cite{liu2017neural}.

Trust in \ac{ai} systems is crucial, particularly in network environments where security, privacy, explainability, and reliability are paramount. In the complex multi-party, multi-network landscape, trust becomes even more challenging due to the increased number of stakeholders and potential attack vectors. 
% Conflict resolution is paramount when multi-party applications control resources over different networks, potentially resulting in inadvertent or malicious conflicts in the assignment of network resources.
The modular nature of the \ac{dmmai} framework supports the multi-party, multi-network vision and enables the quick prototyping of algorithms running in such environments. Therefore, it provides the necessary tools to study trust from three perspectives: 1) identifying attack surfaces in multi-party, multi-network architectures; 2) developing validation and testing methodologies; and 3) ensuring privacy preservation and explainability of \ac{ai} methods. The framework is also envisioned to be easily integrated with existing testbed infrastructures, enabling data collection. This will also facilitate the detection of anomalies in such datasets, which may reveal vulnerabilities and attacks more rapidly and reliably. 

\vspace{-1em}



==> sections/4-research_challenges.tex <==
\section{Research Challenges}
As previously highlighted, 6G networks are not just about faster data transfer anymore. They are set to be adaptive compute-and-communicate systems. The \ac{dmmai} framework's flexibility allows easy integration with existing orchestration frameworks in different network domains and enables practical experiments and use-case studies. However, this flexibility opens up new research questions. 
% We are looking at networks go beyond transferring data -- they are expected to process and make decisions, adapting to ever-changing user needs and environments. 
This section aims to unpack these complex challenges, focusing on how the \ac{dmmai} framework prepares us for the multi-functional and dynamic nature of future 6G networks.

\subsubsection{Orchestration of AI Controllers} A fundamental aspect of the \ac{dmmai} framework is the orchestration of different \ac{ai} controllers to support both user and network services. This orchestration is heavily reliant on the management and curation of data and models across various network environments. It requires an understanding of how to harmonize these controllers end-to-end to support 6G network functions. The orchestration processes will focus on adopting a modern, modular, and cloud-based implementation that can be deployed in a cloud-native environment enabled to interact with all the other elements, e.g., the \acp{ric}, transport \ac{sdn}, and \ac{nos}.

\subsubsection{Decentralized AI Network Operations} 
Our framework serves as a foundational structure for studying decentralized \ac{ai} operations across multiple network platforms. This includes the integration of \acp{aic} within software-defined networking environments, such as near-\ac{rt} and non-\ac{rt} \acp{ric}, \ac{sdn}, and \ac{nos}. It aims to provide a cohesive framework for investigating research topics related to AI in network operations.

\subsubsection{Energy Efficiency in AI and Communications}
Addressing energy efficiency is a critical challenge for the \ac{dmmai} framework. This requires clarifying the energy cost by developing energy models for \ac{ai} operations/computation, sensing, and communication, as well as the energy harvesting aspects. 
% Designing an energy-efficient protocol and optimizing the energy consumption of \ac{ai} and communication systems in 6G networks, while considering key constraints such as timing and data relevance is a priority. 
\ac{dmmai} aims to minimize energy usage in decentralized \ac{ai} setups, ensuring that resources do not operate at full capacity during idle periods.
    
\subsubsection{Complexity and Scale Management} 
The \ac{dmmai} framework is integral to managing the complexity and scale of future 6G networks. It addresses various challenges, including \ac{ai} control plane coordination across different network technologies and domains, end-to-end data management and curation with quality-aware compression~\cite{DBLP:conf/icde/JensenP021}. 
% Here, development of interconnected \acp{aic} is a key innovation.

\subsubsection{AIaaS Integration and Data Curation} 
% The framework also focuses on defining and implementing a modular and cloud-based \ac{aic} framework, which interacts with \ac{ric} and \ac{sdn} controllers. 
The \ac{dmmai} framework involves specifying and implementing interfaces for inter-communication among various \ac{aic} instances, developing capabilities for optical \ac{aic} and inter-\ac{aic} optical-radio communication, and designing data curation functions. It is also crucial for defining and implementing workflows to facilitate the training and deployment of \ac{ai}/\ac{ml} models in \ac{aiaas} setups. 

\subsubsection{Data Collection and AI Foundation Model Research} 
A critical challenge that can be addressed with the \ac{dmmai} framework is efficiently collecting and processing vast, diverse data essential for \ac{ai} foundation model research in 6G networks. This involves not only gathering data from multiple network sources but also ensuring its quality for developing scalable \ac{ai} models. These models are fundamental for various intelligent network functions and must be computationally efficient and adaptable to the dynamic nature of 6G environments. Additionally, the framework must address data governance, ensuring privacy, security, and ethical \ac{ai} practices. This encompasses managing data bias and maintaining model transparency and accountability.

\jinfeng{
\subsubsection{Validation, Dissemination, and Standardization}
It is critical to enable efficient and scalable inter-working and interoperability of AI/ML-based technologies in the multi-party eco-system of telecommunication systems while targeting 6G use cases and deployments. Validation and demonstrations of interoperability, preferably participated by and disseminated to main stakeholders such as operators, equipment, device and application vendors, shall pave the way for global standardization of AI-native networks as they iron out important issues such as training data sharing, model sharing/adaptations/versioning, reference models based minimum performance guarantees, and associated signaling etc. that the standardization must tackle.
}

\vspace{-0.5em}
